RoboCopilot: Human-in-the-loop Interactive Imitation Learning for Robot Manipulation

Learning from human demonstration is an effective approach for learning complex manipulation skills. However, existing approaches heavily focus on learning from passive human demonstration data for its simplicity in data collection. Interactive human teaching has appealing theoretical and practical properties, but they are not well supported by existing human-robot interfaces. This paper proposes a novel system that enables seamless control switching between human and an autonomous policy for bi-manual manipulation tasks, enabling more efficient learning of new tasks. This is achieved through a compliant, bilateral teleoperation system. Through simulation and hardware experiments, we demonstrate the value of our system in an interactive human teaching for learning complex bi-manual manipulation skills.

==> figures/example/figure.tex <==
\begin{figure}[h!]
  \centering
  \includegraphics[width=0.99\textwidth]{figures/example/teaser_image2.png}
  \caption{An illustration of our RoboCopilot System. Left: Our full robot hardware system consisting of a 20DOF mobile bimanual robot and a bilateral teleoperation device. The teleoperation system is kinetically similar to the real robot arm, allowing for direct joint mapping to control the arm. Additionally, the bilateral property of our system enables the teleoperation device to synchronize with the follower robot, allowing for human take-over at any time. Right: Example mobile bimanual daily tasks our system is capable of performing under human supervision.}
  \label{fig:envs}
\end{figure}

==> figures/task/figure.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=1.0\textwidth]{figures/task/task.png}
  \caption{Left: A image of the robot placing the beam into the bin. Middle: An illustration of the train and test locations. Green indicates the train object range. The blue tape marks the location of the place bin, which is highlighted in yellow. The 18 total test locations of the beams are marked in pink and orange respectively. Right: A legend 
 of the relevant task items, showing the 8020 aluminium extrusion and the place bin.}
  \label{fig:envs}
\end{figure}

==> figures/teaser/figure.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=1.0\textwidth]{figures/teaser/jam.png}
  \caption{
  TODO
  }
  \label{fig:teaser}
\end{figure}

==> tables/sim.tex <==
\begin{table*}
  \small
  \caption{The success rate of the can and square tasks on the robomimic dataset\cite{mandlekar2021matters} in the low data imitation learning regime. BC-H refers to behaviour cloning from a human demonstration dataset. BC-Policy refers to behavior cloning from an expert trajectory dataset to make fair comparison with our method. Continual DAgger is our method that continually finetuing with interaction data. We see our continual learning method significantly improves over the baselines.}
  \label{tab:sim_result}
  \centering
  \begin{tabular}{c c c c c}
    \toprule
Environment & \#Demonstrations &      BC-H &        BC-Policy & Continual DAgger (Ours) \\
    \midrule
Can & 20 & 0.61±0.04 & 0.62±0.02 & \textbf{0.67±0.02} \\
Can & 40 & 0.83±0.03 & \textbf{0.93±0.01} & 0.90±0.04 \\
Square & 20 & 0.38±0.02 & 0.41±0.03 & \textbf{0.46±0.02} \\
Square & 40 & 0.52±0.01 & 0.48±0.01 & \textbf{0.56±0.06} \\
    \bottomrule
  \end{tabular}
\end{table*}
